How Language Models Prioritize Contextual Grammatical Cues?

Transformer-based language models have shown an excellent ability to effectively capture and utilize contextual information. Although various analysis techniques have been used to quantify and trace the contribution of single contextual cues to a target task such as subject-verb agreement or coreference resolution, scenarios in which multiple relevant cues are available in the context remain underexplored. In this paper, we investigate how language models handle gender agreement when multiple gender cue words are present, each capable of independently disambiguating a target gender pronoun. We analyze two widely used Transformer-based models: BERT, an encoder-based, and GPT-2, a decoder-based model. Our analysis employs two complementary approaches: context mixing analysis, which tracks information flow within the model, and a variant of activation patching, which measures the impact of cues on the model's prediction. We find that BERT tends to prioritize the first cue in the context to form both the target word representations and the model's prediction, while GPT-2 relies more on the final cue. Our findings reveal striking differences in how encoder-based and decoder-based models prioritize and use contextual information for their predictions.

==> CM.tex <==
Transformers, in general, perform well at retrieving information from any part of the context to build contextualized representations. Our first step is to trace the flow of information within the model to understand how different contextual cues shape the representation of target words. 

This can be achieved using a group of analytical approaches known as `\emph{context-mixing}' methods. These methods provide a map score that quantifies token-to-token interactions at each layer of the model. Although self-attention weights are often seen as a straightforward measure of context mixing in Transformers, numerous studies have shown that relying solely on raw attention can be misleading \citep{bibal-etal-2022-attention, hassid-etal-2022-much}. 
They often focus on meaningless and frequently occurring tokens in the input, such as punctuation marks and special separator tokens in models trained on text \citep{clark-etal-2019-bert}, or background pixels in vision Transformers \citep{Bondarenko2023QuantizableTR}.\footnote{See \citet{kobayashi-etal-2020-attention}'s study for an explanation.} Hence, several methods have been developed to broaden the scope of analysis and incorporate other model components into the computation of the context-mixing \citep{Abnar2020QuantifyingAF, kobayashi-etal-2020-attention, Kobayashi2021IncorporatingRA, ferrando-etal-2022-measuring, modarressi-etal-2022-globenc, mohebbi-etal-2023-quantifying}.

\subsection{Setup}
We use Value Zeroing \citep{mohebbi-etal-2023-quantifying}, a new technique that has shown promise in various domains, including text and speech \citep{mohebbi-etal-2023-homophone}.\footnote{Results for other existing methods can be found in the appendix; while, Attention-Norm \citep{kobayashi-etal-2020-attention} yields results consistent with Value Zeroing, self-attention and Attention Rollout \citep{Abnar2020QuantifyingAF} show a random pattern, confirming the inefficacy of raw attention weights.} It iteratively zeroes out the value vector of each token in the context and measures the cosine distance between the modified and original representation of the target word. This distance indicates the degree each token influences the target word's representation---the greater the distance, the higher the contribution.
Using this method, we extract the contribution of each cue word to the representation of the target word at each layer of the model.\footnote{If a word is split into multiple tokens by the model's tokenizer, we take the maximum score among them.} Scores are normalized to sum to 1 for each context. In encoder-based models, the target position corresponds to the time step of the masked position, while in decoder-based models, it corresponds to the time step when the target token is being generated.

\subsection{Results}
Figures \ref{} and \ref{} demonstrate the contribution of cues to the representation of target words in BERT and GPT-2 models, respectively, averaged across all examples in the test set. The analysis covers both their pre-trained and fine-tuned setups across three scenarios when there are 2, 4, and 6 cues in the context\footnote{Results for other numbers of cues can be found in the appendix.}. 
Additionally, we report the average context mixing score of non-cue tokens in the context, as a baseline, to highlight the significance of the cues' contributions.

As shown in Figure \ref{}, BERT significantly incorporates the cue words into the representation of the target words, starting from the middle layers. Looking at different scenarios when the number of cues in the context increases, the model pays more attention to the first cue. This suggests that the model tends to keep the first cue in the context as the main source of information for gender identification during the information-mixing process. Fine-tuning amplifies the importance of the first cue.

The pattern observed in decoder-based models, however, is clearly different. 
As illustrated in Figure \ref{}, GPT-2 significantly attends to the last cue word in the context, starting from the earlier layers and peaking in the layers closer to the final layer. The later cues make more contributions. Fine-tuning further intensifies this behavior by increasing the importance of the last cue word.

==> Ex_setup.tex <==
In this section, we describe the data and models that we used to set up our experiments.

\subsection{Data}
To measure how the model prioritizes possible cue words within a given context, we need a corpus that includes a diverse range of cue words, each capable of independently disambiguating the target words. We find Biography datasets an ideal case study for this purpose since they naturally describe a single individual, frequently referring to the same subject using referential expressions like pronouns.

We use the test set from the WikiBio \citep{Lebret2016NeuralTG} dataset\footnote{\url{https://huggingface.co/datasets/michaelauli/wiki_bio}}, which contains biographies extracted from Wikipedia with varying lengths. We clean the dataset by removing HTML tags and automatically annotate the cue words in the context by defining a comprehensive list of gender-specific nouns (e.g., `actor'/`actress') and gendered pronouns (e.g., `he'/`she') that serve as cue words. The complete list of potential cue words for identifying gender is presented in Table \ref{tab:list_of_cue_words}.
We then categorize our data based on the number of cue words within the context of each example (ranging from 2 to 6), balance the data through undersampling, and then split it into training and test sets. The training set is used solely for fine-tuning the models, while the test set is used for conducting all our experiments. The statistics for the final dataset are provided in Table \ref{tab:dataset_dist}.

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lc}
        \toprule
        \textbf{Gender} & \textbf{Words} \\
        \midrule
        \multirow{4}{*}{Male} & he, his, him, himself \\
        & master, mister, mr, sir, sire, gentleman, lord \\
        & man, actor, prince, waiter, king \\
        & father, dad, husband, brother, nephew, boy, uncle, son, grandfather \\
        \midrule
        \multirow{4}{*}{Female} & she, her, hers, herself \\
        & miss, ms, mrs, mistress, madam, ma'am, dame \\
        & woman, actress, princess, waitress, queen \\
        & mother, mom, wife, sister, niece, girl, aunt, daughter, grandmother \\
        \bottomrule
    \end{tabular}
    }
    \caption{List of potential cues for gender identification.}
    \label{tab:list_of_cue_words}
\end{table}

\subsection{Target models}
In our experiments, we investigate both encoder-based and decoder-based Transformer \cite{Vaswani2017AttentionIA} language models.
Encoder-based models are trained using masked language modeling, where a certain number of tokens are masked in the input, and the model learns to predict them using bidirectional access to the context.
In contrast, decoder-based models are trained autoregressively to predict the next word in the context by conditioning to only the preceding words.
This distinction allows us to study how different training objectives influence the way models utilize contextual cues.

We opt for BERT \citep{Devlin2019BERTPO} and GPT-2 \citep{radford2019language} as widely used representative models of each category and analyze them in both pre-trained and fine-tuned setups. 
We also replicate our experiments on Gemma \citep{Mesnard2024GemmaOM}, a newly released large language model, in a pre-trained setup only (due to budget constraints). The results are consistent with those of GPT-2, so we report in the appendix.
For fine-tuning, we employ prompt-based fine-tuning \citep{schick-schutze-2021-exploiting, karimi-mahabadi-etal-2022-prompt} by calculating the Cross-Entropy loss specifically over the output logits corresponding to a limited set of vocabulary words, particularly male and female pronouns. The model accuracy before and after fine-tuning is presented in Table \ref{}. \red{table}

\subsection{Model input setup}
Consider the following example from the dataset, which includes four cue words marked with underlines:
% ``\emph{\underline{Ron} \underline{Masak} is an American \underline{actor}. \underline{He} began as a stage performer, and much of \textbf{his} work is in theater.}''
\[
\begin{passage}
\small \underline{Ron} \underline{Masak} is an American \underline{actor}. \underline{He} began as a stage \mbox{performer}, and much of \textbf{his} work is in theater.
\end{passage}
\]
We ask the model to predict the word '\emph{his}' as the target word. So, for an encoder-based model, we replace the target word with a special mask token\footnote{The symbol for the masked token depends on the tokenizer used by the model; for BERT, it is [MASK].}:
\[
\begin{passage}
\small Ron Masak is an American actor. He began as a stage performer, and much of \mask{} work is in theater.
\end{passage}
\]
For a decoder-based model, yet we keep the sentence up to the last word before the target word and ask the model for the next token prediction:
\[
\begin{passage}
\small Ron Masak is an American actor. He began as a stage performer, and much of 
\end{passage}
\]
We filter out instances where the target word is a pronoun and the model correctly identifies the target word, ensuring accurate gender identification.\footnote{We consider target words to be correct in both their capitalized and lowercase forms.} In the next section, we investigate the model internals to understand which contextual cues the model relies on to form representations of the target words and make its final predictions.

==> VP.tex <==
In Section \ref{sec:CM}, we quantified context-mixing in the model to assess each cue word's contribution to the contextualized representation of the target word. This analysis reveals how information from these cues is encoded into the target representation. However, it does not show whether this information is actually used during inference when predicting the target token.
The prediction process (masked or next token prediction) in the model is typically performed by a trained language model head which takes the target representation and generates logits for all tokens in the vocabulary. The goal here, in our second step, is to involve the model's prediction in the analysis to investigate how different contextual cue information influences the model's decision. 

To this end, we leverage the concept of activation patching \citep{}, a commonly used method in mechanistic interpretability studies \citep{}, which measures the drop in a model's confidence using a contrastive approach. The central idea is to overwrite certain activations in the model during a normal run with cached activations obtained from another run on the same example with minimal changes (known as a corrupted run) and observe the impact on the model’s output. While this method has often been used to identify circuits within the model, we employ it here to measure token importance for the model's predictions.

\subsection{Setup}
Activation patching can be applied to various components of a model, including attention heads, MLP outputs, and residual streams. In this study, however, the focus is on patching value vectors within a Transformer layer.
The reason for this choice is to keep the pattern of attention, thus the flow of information, in the model intact, and only nullify the value of a specific cue token representation in a given context.\footnote{Replacing a token from a clean run with one from a corrupted run adds confounding variables, as it introduces a different pattern of attention that may not match those of the clean run.}

We treat the original text in the dataset as clean text and generate corrupted text by replacing all cue words in the clean text with their gender-opposite counterparts. For each cue word, a corresponding counterpart exists, as shown in Table \ref{tab:list_of_cue_words}, except for the first and second cue words, which are first and last names, respectively. In these cases, we substitute the names with a constant name with the opposite gender, ensuring the same number of subwords (see Table \ref{}). \red{a table here}

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        \textbf{Name type} & \textbf{Gender} & \textbf{\#Tokens} & \textbf{Mapping name} \\
        \midrule
        \multirow{4}{*}{First name} 
        & \multirow{2}{*}{Male} & 1 & Bob \\
        &  & 2 & John \\
        & \multirow{2}{*}{Female} & 1 & Amy \\
        &  & 2 & Noora \\
        \midrule
        \multirow{2}{*}{Last name} 
        & \multirow{2}{*}{Both} & 1 & Walker \\
        &  & 2 & Willinsky \\
        \bottomrule
    \end{tabular}
    }
    \caption{List of name mappings}
    \label{tab:list_of_name_mapping}
\end{table}


An example of clean and corrupted text from our dataset is shown below:
\[
\begin{passage}
\small clean:\\ \underline{Ron} \underline{Masak} is an American \underline{actor}. \underline{He} began as a \mbox{stage performer}, and much of \textbf{his} work is in theater.
\end{passage}
\]
\[
\begin{passage}
\small corrupted:\\ \underline{Amy} \underline{Willinsky } is an American \underline{actress}. \underline{She} began as a stage performer, and much of \textbf{her} work is in theater.
\end{passage}
\]

We generate corrupted texts for each example in the test dataset, input them into the model, and cache the resulting value vectors for each token as ``\emph{corrupted value vectors}.''
Subsequently, we input the clean text into the model and record the output probability for the target token ($p_t$).
We then input the clean text again, but this time, we replace the value vector of a specific token at the time step $j$ at a particular layer with its corresponding corrupted value vector and measure the resulting output probability for the target token ($p_t^{\neg j}$). This process is repeated for all tokens across all layers to measure the value patching score: \mbox{$p_t - p_t^{\neg j}$}.
Intuitively, if a cue token is important for the model's prediction, replacing its value vector with a corrupted one (which implies an opposite gender) would lead to a drop in the model's confidence in identifying the true gender.

\subsection{Results}

==> dataModel.tex <==
% Our study required a dataset with specific attributes to address our research question. We aimed to find a corpus that could be restructured to include multiple potential guide tokens, which we call as "cue words." These cue words should be capable of \textbf{independently} predicting a masked pronoun token, enabling the model to accurately infer the masked token using any available cue. 
% A dataset comprising sentences about a single individual was ideal for our purposes, as it naturally contains numerous pronoun references to the same subject. By masking the final pronoun in each sentence, we generate multiple token sources that can correctly predict the masked token, including the subject's first name, last name, gender-specific nouns, other pronouns, and additional contextual identifiers. This approach enables us to investigate the model's ability to utilize various contextual cues for accurate token prediction, aligning with our research objectives.


% \subsection{Dataset} \todo{mention spacy} \todo{add dataset glance in appendix}
% In this paper, \red{we used the WikiBio dataset \citep{Lebret2016NeuralTG}, which contains 728,321 articles from English Wikipedia biography entries}. Each entry includes an infobox with structured data and the corresponding first sentence of the article. 

% This dataset is widely employed for training and evaluating models in generating coherent and contextually relevant biographical text from structured data. \red{We selected this dataset due to its diverse sentences about individuals with varying input lengths, making it suitable for our task of identifying multiple potential cue words to predict a masked pronoun token}. Our unique task of interest can be considered a form of gender agreement task, but with cue words for determining the masked token accessible in multiple tokens.

% To create a more realistic setup, we used the test split of the WikiBio dataset available in Hugging Face \citep{Wolf2019HuggingFacesTS} datasets.\footnote{\url{https://huggingface.co/datasets/michaelauli/wiki_bio}} We then applied several steps to construct our modified dataset. First, we filtered examples to include only those speaking about a single person \red{need to explain how?}. We added the first name and last name of the person as two distinct cue words to our cue words pool for each example.\footnote{Although last names typically lack gender information, we included them as distinct cue words, considering that models may have developed a memorization mechanism for these often-famous individuals encountered during pretraining.} \red{Additionally, We defined numerous gender-specific words, primarily male and female pronouns, along with various honorifics and gender-specific possessional and non-possessional nouns. We iterated over all tokens in each example to identify these potential cue words. The complete list of our potential cue words can be found in Table \ref{tab:gendered_words}.} After identifying all potential cue words that could indicate the individual's gender, we masked the last pronoun (itself a cue word) and ensured no other cue word appeared after the masked token. 

% \begin{table*}
%     \begin{tabular}{lllc}
%         \toprule
%         \textbf{Task type} & \textbf{Example} & \textbf{Cue words} & \textbf{Target word} \\
%         \midrule
%          Masked token prediction & sid kean was a new zealand rugby league player who represented [MASK] country . & \multirow{2}{*}{sid|0|3, kean|4|8} & \multirow{2}{*}{his} \\
%          & Next token prediction & sid kean was a new zealand rugby league player who represented \\
%          \bottomrule
%     \end{tabular}
%     \caption{}
%     \label{tab:dataset_glance}
% \end{table*}


% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{llc}
%         \toprule
%         \textbf{Category} & \textbf{Gender} & \textbf{Words} \\
%         \midrule
%         \multirow{2}{*}{Pronouns} & Male & he, his, him, himself \\
%         & Female & she, her, hers, herself \\
%         \midrule
%         \multirow{2}{*}{Honorifics} & Male & master, mister, mr, sir, sire, gentleman, lord \\
%         & Female & miss, ms, mrs, mistress, madam, ma'am, dame \\
%         \midrule
%         \multirow{2}{*}{Non-Possessionals} & Male & man, actor, prince, waiter, king \\
%         & Female & woman, actress, princess, waitress, queen \\
%         \midrule
%         \multirow{2}{*}{Possessionals} & Male & father, dad, husband, brother, nephew, boy, uncle, son, grandfather \\
%         & Female & mother, mom, wife, sister, niece, girl, aunt, daughter, grandmother \\
%         \bottomrule
%     \end{tabular}
%     \caption{Potential cue words we looked for in every example}
%     \label{tab:gendered_words}
% \end{table*}

% Our reconstructed dataset comprises a masked text, all potential cue words that can independently predict the masked pronoun token, and the target word (the expected token for the model to predict). 
% % An example of each entry of our dataset is shown in Table \ref{}. 
% \red{We split our dataset into train and test sets, using the train set only for fine-tuning the models and the test set for performing all of our experiments. The statistics of our final dataset can be found in Table \ref{tab:dataset_dist}. \todo{move to appendix} We will release our resulting dataset along with our code.} 

% \begin{table}[ht]
%     \centering
%     \resizebox{\columnwidth}{!}{%
%         \begin{tabular}{ccccc}
%             \toprule
%             \textbf{Number of cues} & \textbf{train male} & \textbf{train female} & \textbf{test male} & \textbf{test female} \\
%             \midrule
%             2 & 2088 & 392 & 1377 & 300 \\
%             3 & 1135 & 304 & 693 & 241 \\
%             4 & 716 & 205 & 496 & 133 \\
%             5 & 481 & 157 & 338 & 100 \\
%             6 & 366 & 139 & 217 & 70 \\
%             7 & 306 & 73 & 206 & 61 \\
%             8 & 179 & 67 & 122 & 32 \\
%             9 & 96 & 37 & 81 & 27 \\
%             10 & 63 & 17 & 46 & 5 \\
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{Number of Cues and Gender Distribution \red{we need to make the dataset balanced regarding the number of cues. Maybe excluding 8, 9, and 10, then do undersampling. Also, any need to separate male and female statistics? It's unrelated to our experiment, right? If so, we don't have to separate them here}} 
%     \label{tab:dataset_dist}
% \end{table} 

% \subsection{Models}
% To examine how different kind of models perform the gender agreement task utilizing multiple cues, we will employ two widely used architectures: encoder-based and decoder-based transformers. For the encoder-based models, we will utilize the base versions of BERT \citep{Devlin2019BERTPO} and RoBERTa \citep{Liu2019RoBERTaAR}. To investigate the decoder-based models, we will use GPT2-small \citep{radford2019language} and Gemma-2B \citep{Mesnard2024GemmaOM} model. This selection of models enables a comprehensive comparison of different architectural approaches to the task at hand.

==> discussions.tex <==
% adhere that our analysis is course grained not fine grained

==> eval_1.tex <==
% Context mixing methods analyze how information from different input tokens is combined within Transformer-based models. These methods quantify and visualize each token's contribution to the final representation of a target token. The main objectives include tracing information flow, quantifying token interactions, interpreting model behavior by identifying influential context tokens, evaluating attention mechanisms, and enhancing model interpretability. \red{These methods range from analyzing raw attention weights to using complex techniques that integrate multiple components of the Transformer architecture.}

% We aim to investigate how the representation of the Mask token in encoder-based models and the End token in decoder-based models evolves through subsequent layers. \red{Specifically, we want to determine which cue words are used in each layer to construct the target token's representation. This investigation will reveal how different models perform when multiple sources can be used for a task.}

% In this paper, we employ four context mixing methods, from basic attention weights to more recent, faithful approaches. 
% \vspace{0.5em}
% \newline
% \textbf{Attention weights:} raw attention weights between each pair of tokens within the attention mechanism of a Transformer model. These scores are the simplest and most naive method for studying token-to-token interactions, as they consider only the multi-head attention mechanism and ignore other layer components such as layer normalization and residual blocks.
% \vspace{0.5em}
% \newline
% \textbf{Attention rollout:} an aggregated method for approximating the attention flow based on raw attention weights \citep{Abnar2020QuantifyingAF}. This approach also disregards layer normalization and residual blocks, but by aggregating the scores across subsequent layers, it is argued to provide more faithful context mixing scores.
% \vspace{0.5em}
% \newline
% \textbf{Attention norm:} the extended norm-based method, introduced by \citealp{Kobayashi2021IncorporatingRA}, integrates the norm of transformed input vectors to compute context mixing scores. This approach benefits from incorporating layer normalization and residual blocks, resulting in more accurate scores.
% \vspace{0.5em}
% \newline
% \textbf{Value Zeroing:} aims to measure token interactions by incorporating all components of each encoder layer \citep{mohebbi-etal-2023-quantifying}. To determine how much the target token relies on other tokens to build its representation in each transformer layer, Value Zeroing proposes nullifying the value vector of other tokens individually and computing the resulting representation. A pairwise distance metric is then used to measure the impact of each token's exclusion on the output representation of the target token:
% \begin{equation}
% C_{j} = \tilde{t}^{\neg j} \ast \tilde{t}
% \label{eq:vz}
% \end{equation}
% Where $\tilde{t}$ represents the target token's output representation after processing through a transformer layer, $\tilde{t}^{\neg j}$ represents the target token's output with the value vector of token $j$ set to zero, and $C_{j}$ is the context mixing score for token $j$ in computing the target token's representation. The operation $\ast$ can be any pairwise distance metric, though cosine distance is typically used.

% A key advantage of Value Zeroing is its computation from the transformer layer outputs, which inherently incorporates all components within a layer.
% % including multi-head attention, residual connections, layer normalization, and even feed-forward networks. This approach yields a more robust and reliable context mixing score compared to previous methods.
% \footnote{While Value Zeroing was originally introduced for encoder-based models, we have adapted and implemented it for decoder-based models to suit the requirements of our study, as the process is nearly identical.}

% \subsection{Setup}
% Our resulting dataset contains examples with varying numbers of cue words, ranging from 2 to 6 cues. The primary method involves selecting examples with the same number of cue words and using the masked text as input for transformer models. We then extract four distinct context mixing scores for the target token. In this context, the target token is the final pronoun in the example: represented by the mask token in encoder-based models and by the next token in decoder-based models.

% For instance, consider the example, \textit{"ron masak
% is an american actor. he began as a stage performer, and much of his work is in theater."} Here, we replace the target word, \textit{'his'}, with the mask token. The resulting text is then fed into the encoder-based models. Conversely, for decoder-based models, we remove the target word and all subsequent tokens, and the resulting text is fed into the models. As we ensured that no cue words exist after the last pronoun in each example, removing the subsequent tokens does not affect the model's performance in this specific task.

% We conduct experiments on both pre-trained and fine-tuned versions of each model. Including a fine-tuned model in our analysis provides complementary insights into the importance of cue words, as fine-tuning allows the model to focus on the most relevant words for our task and ensures that target word representations consider the cue words. We utilize prompt fine-tuning \citep{schick-schutze-2021-exploiting, karimi-mahabadi-etal-2022-prompt} and compute Cross Entropy loss solely over the output logits corresponding to all eight male and female pronouns. The accuracy of the models, both before and after fine-tuning, is presented in Table \ref{}. \todo{add table for accuracy}

\begin{figure*}[ht]
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/bert-base-uncased_valueZeroing_2.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/bert-base-uncased_valueZeroing_4.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/bert-base-uncased_valueZeroing_6.pdf}
% \caption{Context mixing scores with 10 cues}
% \label{fig}
\end{subfigure}
\caption{Value Zeroing context mixing scores for the \textbf{pre-trained BERT} model across different numbers of cue words}
\label{fig:bert_cms}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/finetuned-bert_valueZeroing_2.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/finetuned-bert_valueZeroing_4.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/finetuned-bert_valueZeroing_6.pdf}
% \caption{Context mixing scores with 10 cues}
% \label{fig}
\end{subfigure}
\caption{Value Zeroing context mixing scores for the \textbf{fine-tuned BERT} model across different numbers of cue words}
\label{fig:finetuned-bert_cms}
\end{figure*}



% \subsection{Baselines}
% For each context mixing method, we selected the $m^{th}$ row corresponding to the position of the mask token for encoder-based models. For decoder-based models, we selected the last row of the context mixing method. This process yields a 1-D array for each context mixing method. We then extracted the cue word scores\footnote{If a cue word contains multiple tokens, we consider the maximum score among them as the cue word score} and calculated the average score across all examples with the same number of cues.

% To evaluate the significance and effectiveness of cue words in constructing the target token representation at each layer, we employ a simple but intuitive baseline:
% \vspace{0.5em}
% \newline
% \textbf{Non-cue Mean:} This baseline measures the average effectiveness of random non-cue words in constructing the target token representation. The metric is calculated as follows:
% \begin{equation}
% C_{nonCuesMean} = \mathbb{E}_{j \in \{nonCues\}}[\ \tilde{t}^{\neg j} \ast \tilde{t} \ ]
% \end{equation}
% where the notations are consistent with Eq. \ref{eq:vz}. This metric helps us understand the relative importance of cue words compared to random non-cue words. Naturally we expect that, at least in some layers, the cue words context mixing scores will be significantly higher than $C{nonCuesMean}$ due to the nature of our task. This metric also serves as a validation tool for determining the reliability of different context mixing methods.
% \vspace{0.5em}
% \newline
% \textbf{Non-cue Max:} This baseline identifies the maximum context mixing score among non-cue words:
% \begin{equation}
% C_{nonCuesMax} = \max_{j \in {nonCues}}[\ \tilde{t}^{\neg j} \ast \tilde{t} \ ]
% \end{equation}
% This metric indicates whether non-cue words achieve high context mixing scores or not. Hypothesizing the outcome is challenging here, as the model must consider both gender cues and surrounding non-cue words to accurately predict the specific pronoun type, even after determining the correct gender. Nonetheless, it is reasonable to expect cue word scores to be superior to $C_{nonCuesMax}$, especially in the final layers that are critical for the model's final prediction.

% \subsection{Results}
% \todo{mention that we use examples that the model predict the intended target word}
% Figures \ref{fig:bert_cms} and \ref{fig:finetuned-bert_cms} illustrate the Value Zeroing context mixing scores of cue words under three different cue settings for both the pre-trained and fine-tuned BERT models. Given that Value Zeroing provides the most reliable scores among the evaluated context mixing methods, we focus on reporting these results here; the outcomes of other context mixing methods are detailed in Appendix \ref{}. Additionally, results pertaining to the RoBERTa model are presented in Appendix \ref{}. \todo{mention that RoBERTa performs similarly to BERT}

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{figs/relPos_roberta.pdf}
% \caption{Relative position of tokens with maximum context mixing scores for RoBERTa for two cues examples}
% \label{fig:relPos_roberta}
% \end{figure}

% As demonstrated in Figures \ref{fig:bert_cms} and \ref{fig:finetuned-bert_cms}, Value Zeroing effectively highlights the cue words, in contrast to other context mixing methods that fail to do so (see Appendix \ref{}). A consistent pattern is observed across all figures, where cue words significantly influence the last two layers, while the maximum context mixing for non-cue words peaks at layers 2 and 10. Moreover, cue words consistently receive higher scores compared to random non-cue words across nearly all layers. Notably, the fine-tuned BERT model enhances the impact of cue words on constructing target word representations, although this enhancement is not substantial, indicating that the pre-trained model also predominantly utilizes cue words in the last two layers for this task.

% \todo{make y axis of all figures from 0 to 1}
% An intriguing observation is that the BERT model primarily relies on the \textbf{first} and \textbf{last} cue words to determine the gender of the target word, disregarding the intervening cue words regardless of their number. Additionally, the first cue word, which is always the first name, achieves the most significant context mixing score in the last layer, overshadowing even the last cue word. To investigate whether the significance lies in the position as the first cue or as the first name, we replaced the first and last names in all examples with the pronouns \textit{'he'} or \textit{'she'} based on the gender of the example and recalculated the context mixing scores. \todo{add this experiment?}
% \red{Very cool! Let's add them as legends in our figures. So, we'll have two types of cue 1 and 2: cue 1 (first name), cue 2 (last name), cue 1 (pronoun), cue 2 (pronoun)}

% Another notable point is that the last cue word's influence begins to magnify from the middle layers with a relatively constant magnitude, a phenomenon observed across various cue numbers and for both pre-trained and fine-tuned models. We hypothesize that this is primarily due to the proximity of the last cue word to the target word, rather than its informational content regarding gender. This hypothesis is supported by the observation that the last cue word's score is not significantly different from $C_{nonCuesMax}$. Conversely, in the last layer, the first cue word emerges as the dominant token, surpassing other tokens in score. Based on these observations, we conclude that BERT predominantly uses the first cue word/first name in the last two layers to determine the gender of each example. \todo{any further discussion/implication?}

% However, a pertinent question arises: if the model does not utilize the cue words to construct the target word representation in the first 10 layers, then which tokens does it rely on? It is evident that the model must predict the appropriate pronoun type (\textit{subject}, \textit{possessive}, \textit{object}, \textit{reflexive}). We hypothesize that BERT identifies the pronoun type in the early layers and determines the gender in the last two layers to finalize its prediction. To test this hypothesis, we examined the relative position of the token with the maximum context mixing score at each layer, averaged across all examples using two cue words (Figure \ref{fig:relPos_roberta}). We concentrated on examples containing two cue words, ensuring that if the model accurately predicts the gender, the maximum context mixing score should be located at the initial positions of the input, as the cue words are always the first two words in these cases. The results indicate that the highest scoring token in layers 1-10 is consistently located near the [MASK] token position, which may support our hypothesis since predicting the correct pronoun type can be accomplished using the tokens proximal to the target word. Furthermore, in the last two layers, the model's focus shifts dramatically towards the initial positions of the example, suggesting an effort to retrieve the gender information using the two adjacent cue words at the start of the example. Although this experiment was conducted solely with examples containing two cue words, similar trends were observed in examples with additional cue words.

% \subsection{GPT2-small}
\begin{figure*}[ht]
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/gpt2_valueZeroing_2.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/gpt2_valueZeroing_4.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/gpt2_valueZeroing_6.pdf}
% \caption{Context mixing scores with 10 cues}
% \label{fig}
\end{subfigure}
\caption{Value Zeroing context mixing scores for the \textbf{pre-trained GPT2-small} model across different numbers of cue words}
\label{fig:gpt2_cms}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/finetuned-gpt2_valueZeroing_2.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/finetuned-gpt2_valueZeroing_4.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_cms_figs/finetuned-gpt2_valueZeroing_6.pdf}
% \caption{Context mixing scores with 10 cues}
% \label{fig}
\end{subfigure}
\caption{Value Zeroing context mixing scores for the \textbf{fine-tuned GPT2-small} model across different numbers of cue words}
\label{fig:finetuned-gpt2_cms}
\end{figure*}

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{figs/relative_position_GPT2.pdf}
% \caption{Relative position of tokens with maximum context mixing scores for GPT2-small for two cues examples}
% \label{fig:relPos_gpt2}
% \end{figure}

% Figures \ref{fig:gpt2_cms} and \ref{fig:finetuned-gpt2_cms} present the Value Zeroing context mixing scores for cue words across three distinct cue settings in both the pre-trained and fine-tuned GPT2-small models. Consistent with observations in BERT, a similar pattern is discernible in the pre-trained and fine-tuned models. However, in this case, the representation of the target token in layer 10 exhibits the greatest similarity to the cue words, unlike BERT, where the last two layers were most similar. It is noteworthy that fine-tuning amplifies the scores associated with the cue words, yet the influential cues and layers remain unchanged post fine-tuning, which suggests \textbf{???}.

% An important observation here is that GPT2-small primarily utilizes the representation of the \textbf{last} cue word to determine the target token embedding. \footnote{This is not the case for examples with two cues, where the last cue word is typically a surname, which is not indicative of gender.} This finding is in stark contrast to the results found for encoder-based model BERT, where the first cue was the major contributor to the target token representation. Furthermore, the last cue word is the only cue that receives a noticeable score, indicating that the model bases its decision predominantly on the last cue word, effectively ignoring all other cues, which receive even lower scores than a random non-cue token. Based on these observations, we conclude that GPT2-small mainly relies on the last cue word in layers 9 and 10 to determine the gender of each example.
% Similar to BERT, we investigate the layers in which the maximum score does not belong to cue words, as well as identifying other tokens that contribute to the construction of the target word representation. 
\begin{figure*}[ht]
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/sample/finetuned-BERT_cmSample.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig:bert_vp}
\end{subfigure}
\hspace{0.02\textwidth}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/sample/finetuned-GPT2_cmSample.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig:gpt2_vp}
\end{subfigure}
\caption{Value Zeroing scores for a sample text for fine-tuned models. Cue words are highlighted in bold.}
\label{fig:vpSample}
\end{figure*}


\begin{figure*}[ht]
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/sample/finetuned-BERT_vpSample.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig:bert_vp}
\end{subfigure}
\hspace{0.02\textwidth}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/sample/finetuned-GPT2_vpSample.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig:gpt2_vp}
\end{subfigure}
\caption{Value patching scores for a sample text for fine-tuned models. Cue words are highlighted in bold.}
\label{fig:vpSample}
\end{figure*}
% Figure \ref{fig:relPos_gpt2} illustrates the average relative position of the token with the maximum context mixing score across all layers for examples containing two cue words. The concentration around the target word, which is the last token, suggests that the model may be focusing on identifying the pronoun type, a task that can be achieved mainly using tokens near the target token. Additionally, since fine-tuning caused the pre-trained model's focus to shift to earlier positions in layers 9 and 10, which indeed it needs to, we can assert that these layers are particularly significant for our task, indicating that they are primarily responsible for gender pronoun identification.


==> eval_2.tex <==
% The analysis of context mixing within a model layer seeks to determine the extent to which each token representation in the input context, contributes to constructing a specific token representation at the output of that layer. In essence, it is a method for attributing each token's representation to other tokens. In our previous evaluations, we investigated the target token (mask token in BERT and End token in GPT-2) representations to understand how the models utilize various cue words to form the embedding of the target token at each layer's output. However, this analysis pertains to the internal workings of the model, and the models may or may not use these representations for their prediction. This is due to the presence of a language modeling head at the top of the models, typically a feed-forward network that performs the unembedding at the target token's position. \todo{is it true?!}

% To identify which cue words most effectively influence the model's predictions (beyond merely contributing to the target token's internal representations), we designed an experiment incorporating Activation Patching on the value vectors.

% Activation Patching, also known as Interchange Intervention, Causal Tracing, Resample Ablation, or Causal Mediation Analysis, involves replacing the internal activations of a neural network \citep{Heimersheim2024HowTU}. This technique was first introduced in a factual recall task \citep{Meng2022LocatingAE}. The central idea is to overwrite some activations during a model run with cached activations from a previous run (typically on a different input, known as the corrupted run) and observe the impact on the model’s output. While this method is primarily used to identify influential components of a model in performing a specific task, it can also be employed to determine which tokens contribute most to the logits, an analysis that context mixing alone cannot provide. The strength of this method lies in its basis on causal mediation analysis \citep{Pearl2001DirectAI, Vig2020InvestigatingGB}, addressing concerns about the faithfulness of other methods that attempt to attribute tokens to logits \citep{}.\todo{references???}

% Activation Patching can be applied to different parts of a model, including attention heads, MLP outputs, and residual streams \todo{need for more citation here?}. However, in this paper, we focus on a variant of Activation Patching that replaces the value vectors within the multi-head attention mechanism of a transformer layer, which we refer to as \textbf{Value Patching}. We specifically chose to patch the value vectors instead of the more common approach of patching the residual stream output of layers for two main reasons. First, as we employed Value Zeroing context mixing method in earlier evaluations, it is a more consistent approach to perform patching on the value vectors as well \todo{is it?}. Second, patching only the value vector of a token, rather than the layer output of that token, helps prevent any distributional shift that might occur in the attention mechanism. This concern is valid because, in the corrupted sample, other potential cue words might cause the attention to shift if we simply patch the layer output of each token \todo{explain better?}.

% \subsection{Setup}

% We now describe the procedure used to perform value patching across all examples. For each example in our dataset, we treat the original text as the clean text and then create the corrupted text by replacing all cue words in the clean text with their gender-opposite counterparts. There is a one-to-one relationship between cue words for males and females, as shown in Table \ref{tab:list_of_cue_words}. However, for the first name, which is the first cue word in all examples, we map it to unique first names based on gender. Single-token male first names are mapped to \textbf{\textit{Amy}}, double-token male first names to \textbf{\textit{Noora}}, single-token female first names to \textbf{\textit{Bob}}, and double-token female first names to \textbf{\textit{Aron}}. Single-token last names are mapped to \textbf{\textit{Walker}}, and double-token last names to \textbf{\textit{Willinsky}}.\footnote{These names were selected because they have an equal number of tokens across all tokenizers used in this study.} We excluded examples with more than two tokens in their first or last names, as these names are typically less familiar to the models and may not good candidates to represent genders.

% \begin{figure*}[ht]
% \centering
% \begin{subfigure}{0.3\textwidth}
% \centering
% \includegraphics[width=\linewidth]{figs/all_vps_figs/bert-base-uncased_2.pdf}
% % \caption{Context mixing scores with 2 cues}
% \label{fig
% }
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.3\textwidth}
% \centering
% \includegraphics[width=\linewidth]{figs/all_vps_figs/bert-base-uncased_3.pdf}
% % \caption{Context mixing scores with 6 cues}
% \label{fig
% }
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.3\textwidth}
% \centering
% \includegraphics[width=\linewidth]{figs/all_vps_figs/bert-base-uncased_4.pdf}
% % \caption{Context mixing scores with 10 cues}
% \label{fig
% }
% \end{subfigure}
% \caption{Value patching scores for the \textbf{pre-trained BERT} model across different numbers of cue words}
% \label{fig:gpt2_cms}
% \end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_vps_figs/finetuned-bert_2.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_vps_figs/finetuned-bert_4.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_vps_figs/finetuned-bert_6.pdf}
% \caption{Context mixing scores with 10 cues}
% \label{fig}
\end{subfigure}
\caption{Value patching scores for the \textbf{fine-tuned BERT} model across different numbers of cue words}
\label{fig:finetuned-bert_vps}
\end{figure*}



% \begin{figure*}[ht]
% \centering
% \begin{subfigure}{0.3\textwidth}
% \centering
% \includegraphics[width=\linewidth]{figs/all_vps_figs/gpt2_2.pdf}
% % \caption{Context mixing scores with 2 cues}
% \label{fig
% }
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.3\textwidth}
% \centering
% \includegraphics[width=\linewidth]{figs/all_vps_figs/gpt2_3.pdf}
% % \caption{Context mixing scores with 6 cues}
% \label{fig
% }
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.3\textwidth}
% \centering
% \includegraphics[width=\linewidth]{figs/all_vps_figs/gpt2_4.pdf}
% % \caption{Context mixing scores with 10 cues}
% \label{fig
% }
% \end{subfigure}
% \caption{Value patching scores for the \textbf{pre-trained GPT2-small} model across different numbers of cue words}
% \label{fig:gpt2_cms}
% \end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_vps_figs/finetuned-gpt2_2.pdf}
% \caption{Context mixing scores with 2 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_vps_figs/finetuned-gpt2_4.pdf}
% \caption{Context mixing scores with 6 cues}
% \label{fig}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figs/all_vps_figs/finetuned-gpt2_6.pdf}
% \caption{Context mixing scores with 10 cues}
% \label{fig}
\end{subfigure}
\caption{Value patching scores for the \textbf{fine-tuned GPT2-small} model across different numbers of cue words}
\label{fig:finetuned-gpt2_vps}
\end{figure*}

% For instance, consider the clean text \textit{"ron masak is an american actor. he began as a stage performer, and much of <mask> work is in theater."} with the cue words \textit{"ron", "masak", "actor", "he"} and the target token \textit{"his"}. The corrupted text would be \textit{"amy willinsky is an american actress. she began as a stage performer, and much of <mask> work is in theater."}, which would naturally reduce the probability of the target token \textit{"his"} and increase the probability of the corrupted target token \textit{"her"}. Our primary procedure involves constructing such corrupted texts for each example, feeding them into the models, and caching the value vectors for each token. We then feed the models with the clean text and compute the target token probability (the output of softmax). Finally, we feed the models with the clean text again, but this time we replace the value vector of a specific token with the corresponding value vector from the corrupted run. This process is repeated for all tokens and across all layers, measuring the drop in the target token's probability. Naturally, if a token is important for the model's prediction, replacing the clean value vector with a corrupted one will lead to a drop in the target token's prediction. We quantify this drop as the value patching score for that token.
% % \todo{do we need a figure of illustration for the vp here?}
% \begin{equation}
% S_{j} = Prob(t) - prob(t^{\neg j})
% \label{eq
% }
% \end{equation}
% where $Prob(t)$ is \red{the output probability of the target token when the clean text is fed to the model}, $prob(t^{\neg j})$ is the output probability when the value vector of the token at position $j$ is replaced with the corresponding token from the corrupted text's cached value vectors, and $S_{j}$ is the value patching score for token $j$. We compute this metric for every token position and across all layers.

% \subsection{Results}
% Figure \ref{fig:vpSample} showcases value patching scores obtained for our sample text. We patched value vectors for all the positions and across all the layers, but as we expected naturally just the cue words have affect to the logits, however for GPT2 other tokens have shown effect too. Similar to context mixing scores, BERT uses first and last cue words, and GPT2 uses last cue word more. It is also interesting not only cue word "actor" is helpful for GPT2, but it is shifting target token logit to the opposite gender in most layers. \red{We hypothesize that this is due to the gender unbiased tokens like occupations.}

% We computed value patching scores for all of the examples and averaged them across each layer. Figures \ref{fig:finetuned-bert_vps} and \ref{fig:finetuned-gpt2_vps} show the scores for the cue words for three different cue settings for fined-tuned BERT and GPT2-small. Note that the examples used to extract value patching scores are the exact same as the examples used to extract context mixing scores, resulting a more fair comparison and conclusions. Results for the base models can be seen in Appendix \ref{}. Comparing Figures \ref{fig:finetuned-bert_cms} and \ref{fig:finetuned-bert_vps} yields an interesting finding. While BERT extracts mostly from the first cue and also to some points from the last cues to construct the target token representations across last layers, but it dominantly uses the first cue to predict the target token. In other words, BERT do a good job at identifying cue words relevant to the task of gender prediction, but it ends up of not using all of those cues representations when doing the prediction, it just uses the first cue / first name. \todo{do the ablation exp. to find out}

% There is a much more different behavior in GPT2-small. It extracts mostly from the last cue and also to some points from the other last cues to construct the target token representations across last layers. This behavior is also seen almost in the prediction of the model. GPT2-small relies on more diverse sets of cues for it's predictions, however unlike BERT, it appears to have the least reliance on the first cue which is the first name \todo{ablation study}, suggesting that it prefers latest cues respectively. \todo{mention the figs for 5 and 6 cues}
% \todo{any other analysis?}


==> intro.tex <==
% I'll define target and cue words here by making a running example!
% ron masak is an american actor. he began as a stage performer,
% and much of his work is in theater.
% refer to memorization
% refer to code

